Reliable and Trustworthy Machine Learning for Health Using Dataset Shift Detection

Unpredictable ML model behavior on unseen data, especially in the health domain, raises serious concerns about its safety as repercussions for mistakes can be fatal. In this paper, we explore the feasibility of using state-of-the-art out-of-distribution detectors for reliable and trustworthy diagnostic predictions. We select publicly available deep learning models relating to various health conditions (e.g., skin cancer, lung sound, and Parkinson's disease) using various input data types (e.g., image, audio, and motion data). We demonstrate that these models show unreasonable predictions on out-of-distribution datasets. We show that Mahalanobis distance- and Gram matrices-based out-of-distribution detection methods are able to detect out-of-distribution data with high accuracy for the health models that operate on different modalities. We then translate the out-of-distribution score into a human interpretable CONFIDENCE SCORE to investigate its effect on the users' interaction with health ML applications. Our user study shows that the \textsc{confidence score} helped the participants only trust the results with a high score to make a medical decision and disregard results with a low score. Through this work, we demonstrate that dataset shift is a critical piece of information for high-stake ML applications, such as medical diagnosis and healthcare, to provide reliable and trustworthy predictions to the users.

==> chapters/10.checklist.tex <==
\newpage
\section*{NeurIPS 2021 Paper Checklist}
\subsection*{For all authors...}

\textit{(a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?}

Yes. 

\textit{(b) Have you read the ethics review guidelines and ensured that your paper conforms to them?}

Yes. 

\textit{(c) Did you discuss any potential negative societal impacts of your work?}

Yes. We have added discussion on negative societal impacts in Section~\ref{sec:discussion}.

\textit{(d) Did you describe the limitations of your work?}

Yes. The limitations of the work is discussed in Section~\ref{sec:discussion}

\subsection*{If you are including theoretical results...}

\textit{(a) Did you state the full set of assumptions of all theoretical results?}

N/A.

\textit{(b) Did you include complete proofs of all theoretical results?}

N/A

\subsection*{If you ran experiments...}

\textit{(a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?}

Yes. We have added code, data, and instructions required to reporduce the experiment in Section~\ref{sec:performance-eval-setup} and Section~\ref{sec:ood-setup}.

\textit{(b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?}

Yes. We have added all the training details in Section~\ref{sec:performance-eval-setup} and Section~\ref{sec:ood-setup}.

\textit{(c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?}

Yes. Due to space limitation, we have added a performance evaluation table with standard deviation in Appendix~\ref{sec:model-performance-ci}.


\textit{(d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?}

Yes. We have included computing resources used in this work in Section~\ref{sec:performance-eval-setup}. Some datasets (e.g., MHEALTH, ICBHI 2017) did not specify their license. However, all of them mentioned that the datasets are available for public use.

\subsection*{If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...}

\textit{(a) If your work uses existing assets, did you cite the creators?}

Yes. We have cited and added URLs for all the datasets, code, and pre-trained models in Section~\ref{sec:models-datasets},  Section~\ref{sec:performance-eval-setup}, and Section~\ref{sec:ood-setup}. 

\textit{(b) Did you mention the license of the assets?}

Yes. We have specified license of the datasets in Section~\ref{sec:models-datasets}

\textit{(c) Did you include any new assets either in the supplemental material or as a URL?}

This work does not generate new assets.

\textit{(d) Did you discuss whether and how consent was obtained from people whose data you're using/curating?}

Yes. Face dataset received consents from the participants for the data release and future use. We have added the information in Section~\ref{sec:models-datasets}.

\textit{(e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?}

Yes. Face dataset contains PII. But, all participants gave consents for the images to be used for online study and publication. We have added the information in Section~\ref{sec:models-datasets}.

\subsection*{If you used crowdsourcing or conducted research with human subjects...}

\textit{(a) Did you include the full text of instructions given to participants and screenshots, if applicable?}

Yes. We have added the screenshot of the user study interfaces in Appendix~\ref{sec:user-study-interface}.

\textit{(b) Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?}

Yes. We have added the IRB information in Section~\ref{sec:user-study-procedures} and Appendix~\ref{sec:user-study-interface}

\textit{(c) Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?}

Yes. We have added compensation information in Section~\ref{sec:user-study-procedures}.
